Seg-VAR: Image Segmentation with Visual Autoregressive Modeling

While visual autoregressive modeling (VAR) strategies have shed light on image generation with the autoregressive models, their potential for segmentation, a task that requires precise low-level spatial perception, remains unexplored. Inspired by the multi-scale modeling of classic Mask2Former-based models, we propose Seg-VAR, a novel framework that rethinks segmentation as a conditional autoregressive mask generation problem. This is achieved by replacing the discriminative learning with the latent learning process. Specifically, our method incorporates three core components: (1) an image encoder generating latent priors from input images, (2) a spatial-aware seglat (a latent expression of segmentation mask) encoder that maps segmentation masks into discrete latent tokens using a location-sensitive color mapping to distinguish instances, and (3) a decoder reconstructing masks from these latents. A multi-stage training strategy is introduced: first learning seglat representations via image-seglat joint training, then refining latent transformations, and finally aligning image-encoder-derived latents with seglat distributions. Experiments show Seg-VAR outperforms previous discriminative and generative methods on various segmentation tasks and validation benchmarks. By framing segmentation as a sequential hierarchical prediction task, Seg-VAR opens new avenues for integrating autoregressive reasoning into spatial-aware vision systems. Code will be available at https://github.com/rkzheng99/Seg-VAR.

==> tab/ablation.tex <==
\begin{table}[t]

    \centering
    % \caption{\textbf{Comparison on referring video segmentation and video instance segmentation datasets.} }
    \begin{minipage}{0.32\textwidth}
        \vspace{5pt}
        \label{tab:k&T}
        \resizebox{\linewidth}{!}
        {
            \tablestyle{1.5pt}{1.2}
            \begin{tabular}{lcc}
            \toprule
            Method & Dataset & mIoU \\
            \midrule
            Vanilla VAR &ADE20K & 77.4 \\ 
            Seg-VAR &ADE20K & 85.8 \\
            \bottomrule
          \end{tabular}
        }
        \vspace{5pt}
        \caption{\textbf{Ablation on the key design of {\model}.}  These results demonstrate that simply using vanilla VAR without seglat modules, the result is 8.4 lower than our Seg-VAR.}
        \label{tab:vanila_design}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \vspace{5pt}
        \label{tab:k&T}
        \resizebox{\linewidth}{!}
        {
            \tablestyle{2pt}{1.2}
            \begin{tabular}{lcc}
            \toprule
            Method & Dataset & mIoU \\
            \midrule
            Mask2Former &R50 & 63.8 \\ 
            Seg-VAR &R50 & 64.2 \\  
            \bottomrule
          \end{tabular}
        }
        \vspace{5pt}
        \caption{\textbf{Ablation on the parameters.}  These results demonstrate that under comparable parameters, our Seg-VAR still outperforms Mask2Former in the R50 backbone.}
        \label{tab:parameters}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \scriptsize
        \vspace{5pt}
        \resizebox{\linewidth}{!}
        {
          \tablestyle{1pt}{1.2}
          \begin{tabular}{lc|lc}
            \toprule
            Grid Number & mIoU & Palette Size & mIoU \\
            \midrule
            4 & 84.4 & 124 & 85.4 \\ 
            8 & 85.2 & 215 & 85.8 \\ 
            12 & 85.8 & 342 & 85.3 \\ 
            \bottomrule
          \end{tabular}
          
        }
        \vspace{5pt}
          \caption{\textbf{Ablation on different generation models}. We experimented on different image generation models, the results indicate the superiority of VAR in segmentation tasks.}
          \label{tab:grid}
    \end{minipage}

\end{table}
\vspace{-10pt}

==> tab/ade20k.tex <==
\begin{table}[tb]
\tablestyle{1.8pt}{1.1}
\renewcommand\tabcolsep{7.0pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{lccc|c}
\hline

\hline

Method & Pretrain & Backbone & Iteration &mIoU \\
\hline
\multicolumn{3}{l}{\emph{- Discriminative modeling:}}\\
\hline
\multicolumn{1}{l}{FCN~\cite{long2015fully}}&1K & ResNet-101 & {160k} &{41.40} \\
\multicolumn{1}{l}{CCNet~\cite{huang2019ccnet}}&1K & ResNet-101 & {160k}&{43.71} \\
\multicolumn{1}{l}{DANet~\cite{fu2019dual}}&1K & ResNet-101 &{160k} &  {44.17}\\
\multicolumn{1}{l}{UperNet~\cite{xiao2018unified}}&1K & ResNet-101 & {160k}&  {43.82}\\
\multicolumn{1}{l}{Deeplab-v3+~\cite{chen2018encoder}}&1K & ResNet-101 &{160k} & {45.47}\\
\multicolumn{1}{l}{Maskformer~\cite{cheng2021per}} & 1K& ResNet-101 & {160k}& {45.50}\\
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}} & 1K& ResNet-101 & {160k}& {47.80}\\
\multicolumn{1}{l}{OCRNet~\cite{yuan2019object}}&1K & HRNet-W48 &{160k} &  {43.25}\\
\multicolumn{1}{l}{SegFormer~\cite{xie2021segformer}}&1K & MiT-B5 & {160k}& \textbf{50.08}\\
\multicolumn{1}{l}{SETR~\cite{zheng2021rethinking}}&22K & ViT-Large& {160k}& {48.28}\\
\hline
\multicolumn{3}{l}{\emph{- Generative modeling:}} \\
\hline
\multicolumn{1}{l}{UViM$^\dag$~\cite{kolesnikov2022uvim}} & 22k & Swin-Large & 160k &43.71 \\
\multicolumn{1}{l}{GSS-FF~\cite{chen2023generative}}&22K & Swin-Large & 160k &46.29 \\
\multicolumn{1}{l}{GSS-FW~\cite{chen2023generative}}&22K & Swin-Large & 160k &{48.54} \\
\multicolumn{1}{l}{{\model}}&22K & Swin-Large & 160k &\textbf{54.90} \\

\hline

\hline
\end{tabular}

\caption{\textbf{Semantic Segmentation comparison with previous art methods on the ADE20K {\tt val} split}.  % on PyTorch.
}
\label{tab:ade20k_val}
\end{table}

==> tab/cityscapes.tex <==
\begin{table}[tb]
\tablestyle{1.8pt}{1.1}
\renewcommand\tabcolsep{7.1pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{lccc|c}
\hline

\hline


Method & Pretrain & Backbone & Iteration&mIoU \\
\hline
\multicolumn{4}{l}{\emph{- Discriminative modeling:}} \\
\hline
\multicolumn{1}{l}{FCN~\cite{long2015fully}} & 1K & ResNet-101 & {80k} &{77.02}\\ 
\multicolumn{1}{l}{PSPNet~\cite{zhao2017pyramid}} & 1K& ResNet-101 &{80k}  & {79.77}\\
\multicolumn{1}{l}{DeepLab-v3+~\cite{chen2018encoder}}& 1K & ResNet-101 &{80k} & {80.65}\\

\multicolumn{1}{l}{NonLocal~\cite{wang2018nonlocal}} & 1K& ResNet-101 &{80k} & {79.40}\\
\multicolumn{1}{l}{CCNet~\cite{huang2019ccnet}}& 1K & ResNet-101 &{80k} &{79.45} \\
% \multicolumn{1}{l}{GCNet~\cite{cao2019gcnet}} & 1K& ResNet-101 &{80k} & {} \\
\multicolumn{1}{l}{Maskformer~\cite{cheng2021per}} & 1K& ResNet-101 & {90k} & {78.50} \\ % resnet-101 miou 78.5, resnet-101-c miou 79.70
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}} & 1K& ResNet-101 & {90k} & {80.10} \\ 
\multicolumn{1}{l}{SETR~\cite{zheng2021rethinking}} & 22K& ViT-Large & {80k} & {78.10} \\
\multicolumn{1}{l}{UperNet~\cite{xiao2018unified}}& 22K & Swin-Large & {80k}  & {82.89}\\ % 81.0
% \multicolumn{1}{l}{Maskformer~\cite{cheng2021per}}& 22K & Swin-Large & {90k}  & {78.50}\\
\multicolumn{1}{l}{Mask2former~\cite{cheng2022masked}}& 22K & Swin-Large & {90k}  & \textbf{83.30}\\
\multicolumn{1}{l}{SegFormer~\cite{xie2021segformer}} & 1K& MiT-B5 & {160k} & {82.25} \\
\hline
\multicolumn{3}{l}{\emph{- Generative modeling:}} \\
\hline
\multicolumn{1}{l}{UViM$^\dag$~\cite{kolesnikov2022uvim}}& 22K & Swin-Large & 160k &70.77 \\
\multicolumn{1}{l}{GSS-FF~\cite{chen2023generative}}& 22K & Swin-Large & 80k & {78.9}\\
\multicolumn{1}{l}{GSS-FT-W~\cite{chen2023generative}}& 22K & Swin-Large & 80k & {80.05}\\
\multicolumn{1}{l}{{\model}}& 22K & Swin-Large & 80k & \textbf{84.8}\\

\hline

\hline
\end{tabular}
\caption{\textbf{Semantic Segmentation on the Cityscapes {\tt val} split:} UViM$^\dag$~\cite{kolesnikov2022uvim} is reproduced by us on PyTorch. ``1K" means pretrained on ImageNet 1K~\cite{deng2009imagenet} while ``22K" means pretrained on ImageNet 22K~\cite{deng2009imagenet}.}
\label{tab:cityscapes_val}
\vspace{-0.5em}
\end{table}
